Riemannian Optimization for Distance-Geometric Inverse Kinematics

Solving the inverse kinematics problem is a fundamental challenge in motion planning, control, and calibration for articulated robots. Kinematic models for these robots are typically parametrized by joint angles, generating a complicated mapping between the robot configuration and the end-effector pose. Alternatively, the kinematic model and task constraints can be represented using invariant distances between points attached to the robot. In this paper, we formalize the equivalence of distance-based inverse kinematics and the distance geometry problem for a large class of articulated robots and task constraints. Unlike previous approaches, we use the connection between distance geometry and low-rank matrix completion to find inverse kinematics solutions by completing a partial Euclidean distance matrix through local optimization. Furthermore, we parametrize the space of Euclidean distance matrices with the Riemannian manifold of fixed-rank Gram matrices, allowing us to leverage a variety of mature Riemannian optimization methods. Finally, we show that bound smoothing can be used to generate informed initializations without significant computational overhead, improving convergence. We demonstrate that our inverse kinematics solver achieves higher success rates than traditional techniques, and substantially outperforms them on problems that involve many workspace constraints.

==> tables/planar_chain_old.tex <==
\begin{tabular}{llrrrrr}

 & \textbf{Solver} &  \thead{Success\\Rate} &  \thead{Mean No.\\of Iterations} &  \thead{Mean\\Runtime (s)} &  \thead{Mean Pos.\\Error (m)} & \thead{Mean Rot. \\Error (rad)} \\
\midrule
\multirow{4}{*}{6 DoF Unbounded}
&                   \texttt{trust-exact} &         1.000 &                  26.980 &             0.754 &                0.000 &                  0.000 \\
&                        \texttt{FABRIK} &         1.000 &                   8.960 &             0.011 &                0.000 &                  0.000 \\
&       \texttt{Riem. TR} &         1.000 &                  20.100 &             0.025 &                0.000 &                  0.000 \\
&  \texttt{Riem. TR+BS} &         1.000 &                  12.210 &             0.018 &                0.000 &                  0.000 \\
\cmidrule(r){2-7}
\multirow{4}{*}{6 DoF Bounded}
&                  \texttt{trust-constr} &         0.960 &                  40.390 &             0.537 &                0.000 &                  0.000 \\
&                        \texttt{FABRIK} &         0.100 &                 182.660 &             0.262 &                0.000 &                  0.000 \\
&       \texttt{Riem. TR} &         0.970 &                  27.580 &             0.025 &                0.000 &                  0.000 \\
&  \texttt{Riem. TR+BS} &         0.980 &                  25.980 &             0.024 &                0.000 &                  0.000 \\
\cmidrule(r){2-7}
\multirow{4}{*}{10 DoF Unbounded}
&                   \texttt{trust-exact} &         1.000 &                  28.390 &             1.138 &                0.000 &                  0.000 \\
&                        \texttt{FABRIK} &         1.000 &                   7.760 &             0.014 &                0.000 &                  0.000 \\
&       \texttt{Riem. TR} &         1.000 &                  22.190 &             0.023 &                0.000 &                  0.000 \\
&  \texttt{Riem. TR+BS} &         1.000 &                  12.600 &             0.016 &                0.000 &                  0.000 \\

\cmidrule(r){2-7}
\multirow{4}{*}{10 DoF Bounded}
&                  \texttt{trust-constr} &         1.000 &                  47.890 &             0.918 &                0.000 &                  0.000 \\
&                        \texttt{FABRIK} &         0.510 &                 103.780 &             0.187 &                0.000 &                  0.000 \\
&       \texttt{Riem. TR} &         0.900 &                  46.160 &             0.048 &                0.000 &                  0.000 \\
&  \texttt{Riem. TR+BS} &         1.000 &                  16.300 &             0.017 &                0.000 &                  0.000 \\

\end{tabular}

==> tables/table_2.tex <==
\begin{tabular}{llrrrrrr}

& \textbf{Solver} &  \thead{Success\\Rate} &  \thead{Mean No.\\of Iterations} &  \thead{Mean\\Runtime (s)} &  \thead{Mean\\Error (m)} &  \thead{Std. Dev. \\ Error (m)} & \thead{Max. \\Error (m)} \\
\midrule
\multirow{10}{*}{6 DoF Unbounded}
&                               \texttt{BFGS} &         0.641 &                  20.074 &             0.014 &           0.102 &                0.196 &           1.376 \\
&                                 \texttt{CG} &         0.642 &                  40.982 &             0.043 &           0.103 &                0.197 &           1.631 \\
&                          \texttt{Newton-CG} &         0.645 &                  16.379 &             0.040 &           0.103 &                0.204 &           1.406 \\
&                        \texttt{trust-exact} &         0.719 &                   8.900 &             0.023 &           0.069 &                0.151 &           0.922 \\
&                             \texttt{FABRIK} &         0.562 &                 109.200 &             0.097 &           0.224 &                0.404 &           3.063 \\
&                           \texttt{Jacobian} &         0.000 &                  94.555 &             0.565 &           1.981 &                1.030 &           5.795 \\
&            \texttt{Riem. TR} &         0.676 &                  15.791 &             1.037 &           0.093 &                0.192 &           1.133 \\
&       \texttt{Riem. TR + BS} &         0.680 &                   9.538 &             1.033 &           0.085 &                0.168 &           1.026 \\
&       \texttt{Riem. CG} &         0.661 &                  77.484 &             1.058 &           0.099 &                0.196 &           1.077 \\
&  \texttt{Riem. CG + BS} &         0.669 &                  66.973 &             1.046 &           0.091 &                0.184 &           1.091 \\
\cmidrule(r){2-8}
\multirow{4}{*}{6 DoF Bounded}
&                  \texttt{trust-constr} &         0.934 &                  30.199 &             0.190 &           0.020 &                0.089 &           1.682 \\
&                        \texttt{FABRIK} &         0.867 &                 113.652 &             0.082 &           0.043 &                0.107 &           0.654 \\
&       \texttt{Riem. TR} &         0.941 &                  14.448 &             0.036 &           0.012 &                0.050 &           0.549 \\
&  \texttt{Riem. TR+BS} &         0.939 &                   8.429 &             0.029 &           0.012 &                0.048 &           0.536 \\

\cmidrule(r){2-8}
\multirow{10}{*}{14 DoF Unbounded}
&                               \texttt{BFGS} &         0.213 &                  45.047 &             0.089 &           0.204 &                0.224 &           1.281 \\
&                                 \texttt{CG} &         0.104 &                  99.489 &             0.286 &           0.207 &                0.204 &           1.222 \\
&                          \texttt{Newton-CG} &         0.222 &                  26.036 &             0.269 &           0.200 &                0.218 &           1.193 \\
&                        \texttt{trust-exact} &         0.221 &                  15.394 &             0.149 &           0.194 &                0.213 &           1.403 \\
&                             \texttt{FABRIK} &         0.120 &                 192.335 &             0.312 &           0.491 &                0.515 &           3.154 \\
&                           \texttt{Jacobian} &         0.000 &                  99.828 &             1.169 &           2.731 &                1.139 &           7.217 \\
&            \texttt{Riem. TR} &         0.234 &                  25.748 &             0.093 &           0.202 &                0.238 &           1.695 \\
&       \texttt{Riem. TR + BS} &         0.269 &                  16.596 &             0.082 &           0.172 &                0.201 &           1.038 \\
&       \texttt{Riem. CG} &         0.021 &                  99.000 &             0.049 &           0.265 &                0.240 &           1.699 \\
&  \texttt{Riem. CG + BS} &         0.060 &                  98.996 &             0.049 &           0.200 &                0.192 &           1.330 \\
\cmidrule(r){2-8}
\multirow{4}{*}{14 DoF Bounded}
&                  \texttt{trust-constr} &         0.781 &                 110.522 &             1.670 &           0.107 &                0.234 &           1.697 \\
&                        \texttt{FABRIK} &         0.013 &                 200.000 &             0.449 &           0.687 &                0.286 &           1.469 \\
&       \texttt{Riem. TR} &         0.779 &                  28.450 &             0.160 &           0.021 &                0.081 &           0.767 \\
&  \texttt{Riem. TR+BS} &         0.803 &                  19.914 &             0.165 &           0.019 &                0.082 &           0.791 \\
\cmidrule(r){2-8}
\multirow{4}{*}{30 DoF Bounded}
&                  \texttt{trust-constr} &         0.447 &                 189.575 &             8.775 &           0.370 &                0.438 &           1.835 \\
&                        \texttt{FABRIK} &         0.000 &                 200.000 &             1.182 &           1.102 &                0.235 &           2.193 \\
&       \texttt{Riem. TR} &         0.501 &                  71.138 &             1.134 &           0.029 &                0.076 &           0.561 \\
&  \texttt{Riem. TR+BS} &         0.622 &                  61.846 &             1.222 &           0.027 &                0.068 &           0.561 \\


\end{tabular}


==> tables/table_3.tex <==
\begin{tabular}{llrrrrrr}

& \textbf{Solver} &  \thead{Success\\Rate} &  \thead{Mean No.\\of Iterations} &  \thead{Mean\\Runtime (s)} &  \thead{Mean\\Error (m)} & \thead{Std. Dev. \\ Error (m)} & \thead{Max. \\Error (m)} \\
\midrule
\multirow{10}{*}{6 DoF Unbounded}
&                               \texttt{BFGS} &         0.987 &                  72.889 &             0.399 &           0.001 &                0.003 &           0.045 \\
&                                 \texttt{CG} &         0.400 &                  99.437 &             0.828 &           0.025 &                0.036 &           0.360 \\
&                          \texttt{Newton-CG} &         0.937 &                  59.252 &             2.247 &           0.003 &                0.015 &           0.394 \\
&                        \texttt{trust-exact} &         1.000 &                  32.444 &             1.105 &           0.000 &                0.000 &           0.001 \\
&                             \texttt{FABRIK} &         0.000 &                 200.000 &             0.202 &           2.131 &                0.232 &           3.198 \\
&            \texttt{Riem. TR} &         1.000 &                  23.846 &             0.111 &           0.000 &                0.000 &           0.000 \\
&       \texttt{Riem. TR + BS} &         1.000 &                  18.425 &             0.108 &           0.000 &                0.000 &           0.000 \\
&       \texttt{Riem. CG} &         0.378 &                  98.631 &             0.049 &           0.028 &                0.131 &           2.962 \\
&  \texttt{Riem. CG + BS} &         0.455 &                  99.000 &             0.050 &           0.020 &                0.041 &           0.878 \\
\cmidrule(r){2-8}
\multirow{10}{*}{6 DoF Bounded}
&                           \texttt{L-BFGS-B} &         0.551 &                  51.168 &             0.278 &           0.046 &                0.184 &           2.325 \\
&                                \texttt{TNC} &         0.509 &                  17.100 &             0.454 &           0.048 &                0.155 &           2.260 \\
&                              \texttt{SLSQP} &         0.752 &                  35.522 &             0.182 &           0.012 &                0.043 &           0.844 \\
&                       \texttt{trust-constr} &         0.971 &                  71.795 &             2.121 &           0.003 &                0.040 &           1.121 \\
&                             \texttt{FABRIK} &         0.000 &                 200.000 &             0.198 &           2.131 &                0.232 &           3.198 \\
&            \texttt{Riem. TR} &         0.995 &                  23.661 &             0.113 &           0.000 &                0.000 &           0.000 \\
&       \texttt{Riem. TR + BS} &         0.983 &                  18.346 &             0.109 &           0.000 &                0.013 &           0.394 \\
&       \texttt{Riem. CG} &         0.353 &                  98.899 &             0.050 &           0.020 &                0.029 &           0.366 \\
&  \texttt{Riem. CG + BS} &         0.425 &                  99.000 &             0.050 &           0.020 &                0.041 &           0.877 \\
\end{tabular}

